The Dynamics of Vehicular Networks in Urban Environments

Vehicular Ad hoc NETworks (VANETs) have emerged as a platform to support intelligent inter-vehicle communication and improve traffic safety and performance. The road-constrained, high mobility of vehicles, their unbounded power source, and the emergence of roadside wireless infrastructures make VANETs a challenging research topic. A key to the development of protocols for inter-vehicle communication and services lies in the knowledge of the topological characteristics of the VANET communication graph. This paper explores the dynamics of VANETs in urban environments and investigates the impact of these findings in the design of VANET routing protocols. Using both real and realistic mobility traces, we study the networking shape of VANETs under different transmission and market penetration ranges. Given that a number of RSUs have to be deployed for disseminating information to vehicles in an urban area, we also study their impact on vehicular connectivity. Through extensive simulations we investigate the performance of VANET routing protocols by exploiting the knowledge of VANET graphs analysis.

==> figures.tex <==
\section{SF}
 	\subsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{SF}
 	\subsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/SF/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{NY}
 	\subsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{NY}
 	\subsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/BC/bcentrality}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{LA}
 	\subsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{LA}
 	\subsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{LA HD}
 	\subsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{LA HD}
 	\subsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/Degree/Degree}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/DegreeDistr/DegreeDistr}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_HD/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{NY with RSU}
 	\subsection{RSU Granularity: 3rsuPerKm2 }
 		\subsubsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 3rsuPerKm2 }
 		\subsubsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 1rsuPerKm2 }
 		\subsubsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 1rsuPerKm2 }
 		\subsubsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 2rsuPerKm2 }
 		\subsubsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 2rsuPerKm2 }
 		\subsubsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/NY_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
\section{LA with RSU}
 	\subsection{RSU Granularity: 3rsuPerKm2 }
 		\subsubsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 3rsuPerKm2 }
 		\subsubsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/3rsuPerKm2/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 1rsuPerKm2 }
 		\subsubsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 1rsuPerKm2 }
 		\subsubsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/1rsuPerKm2/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 2rsuPerKm2 }
 		\subsubsection{TX Range: 300 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/300/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage
 	\subsection{RSU Granularity: 2rsuPerKm2 }
 		\subsubsection{TX Range: 75 m}
		\begin{figure*}[h]
		\centering
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/90PercDiameter/90PercDiameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/AvgDegreeSeparat/AvgDegreeSeparat}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/BC/BC}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/ClustCoeff/ClustCoeff}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Clusters/Clusters}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/CommModularity/CommModularity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Communities/Communities}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Diameter/Diameter}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/GraphDensity/GraphDensity}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/LobbyIndex/LobbyIndex}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/NodesInBiggestCluster/NodesInBiggestCluster}}
\subfigure{\includegraphics[width=0.32\textwidth]{/home/nickl/Desktop/ExtFigures/LA_wRSU/2rsuPerKm2/graphDumps/75/FiguresFromNET/Triangles/Triangles}}
				\end{figure*}
\clearpage


==> implications.tex <==
\section{Implications}
\label{sec-implications}
In the previous section we conducted a thorough analysis of the topological
characteristics of a large-scale VANET graph and gained a deep understanding of
its shape. The question that remains to be answered is whether this information
is useful from an engineering perspective. In the next paragraphs, we identify
how existing routing protocols for VANETs can be enhanced, providing significant
perspectives and insights.


\subsection{Network-oriented metrics}

Recently, researchers have realized the importance of exploiting vehicle traffic
density in designing efficient and reliable information dissemination protocols.
In~\cite{Resta2007} authors established a rigorous theoretical framework and
pointed out that an optimal message forwarding strategy is partly determined by
the vehicle density of underlying VANETs. Based on our observations, the
vehicle's density is quite large in urban environments. Therefore, protocols
based on flooding will choke the network; thus, topology control algorithms are
necessary.

Other sound observations are that 1) the VANET exhibits small world properties
and 2) the degree distribution of VANETs is skewed. These observations are
useful since they provide indications about the richness of the network
connectivity. Specifically, VANETs have a small diameter, exhibit high
clustering and their degree distribution is characterized by a power-law
behavior. Therefore, gossip protocols~\cite{Boyd2006} should be investigated in
order to take advantage of small-world properties, and especially scale-free
ones, in order to efficiently disseminate information in vehicular networks.



%, providing answers to the key question:
%``how many available paths exist between vehicles?''. This statistic provides an
%indication about how many duplicate messages will be received at a vehicle,
%implying how severe the broadcast storm problem is for critical safety
%applications.

In addition, the network's density makes the use of power transmission adjustment
mandatory. The difference in a VANET setting is that this procedure must be {\it
continuous}, and can not be decided once in advance. Such continuous power
adjustment is not easy to achieve, unless it is done on a per-road-segment basis (e.g., CVIS platform),
i.e., decide power transmission levels for segments of the roads, based on
observed vehicle density (i.e., in places where vehicles' communities exist). How
to segment the roads, is a matter of investigation.


\subsection{Cluster analysis metrics}
The existence of communities implies that mobility models like the Random Way
Point, which are based on types of random walks should be abandoned, because they
do not produce clusterings of the vehicles and additionally they do not support
the existence of ``hub" vehicles that explain the distributions of the centrality
metrics. Therefore, research towards richer models (e.g., \cite{Musolesi2007})
must be conducted. Specifically, vehicles that belong in a community act as a
``data island''. This is widely observed in highways, where opportunistic
protocols are used (e.g., Opportunistic Packet Relaying protocol -
OPERA~\cite{Abuelela2008}). Therefore, since we also observe communities in urban
environments, such protocols could also be applied in urban environments.
Furthermore, the existence of communities implies also that leader election
algorithms will work successfully~\cite{Raya2006}, especially if we incorporate
the centrality metrics in their selection.


In addition, the existence of communities contributes on addressing the Maximum
Coverage Problem~\cite{Trullols2010}. Considering an area with an arbitrary road
topology that must be equipped with a limited number k of RSUs, where to place
them so as to maximize the dissemination of information? In points where borders
of clusters exist, or in places where vehicle communities exist. Similarly,
installation of RSUs is suggested in places where the nodes have low localized
clustering coefficient (sparse network), and thus the delivery of messages would
require a significant amount of time without the infrastructure.

\subsection{Centrality metrics}
Article~\cite{Erramilli2008} asked the question: which nodes will be the
forwarders in routing? Our study is able to provide an answer to this: we can
draw such nodes among those with high centrality value. These nodes are also
perfect candidates for message ferrying in case of network partitionings.
Similarly, for geocasting applications, nodes with high lobby index are ideal for
carrying out the rebroadcasts so as to spread the message to many recipients
with as few rebroadcasts as possible.

Moreover, for applications requiring awareness of the positions of other vehicles
through periodic beacons, or the distribution of traffic related data through
periodic beacons, the exploitation of the more ``central" vehicles for these
tasks could relieve the network from redundant broadcasts and reduce the
collisions.


Finally, the high mobility of the vehicles, make graph-based topology-control
methods (spanning trees, Ga\-briel/Yao graph, RNG) not appealing; clustering is
preferable. Which could be the clusterheads? Not necessarily high-degree nodes,
but those with large betweenness centrality (if we need a few clusters), or those
with high lobby centrality (if we need a lot of clusters).


\subsection{Link Level metrics}

The number of connected periods is a critical statistic since it implies how
often a protocol needs to re-initiate route discovery process. Similarly, the
duration of connected periods is important for designing a routing protocol,
since several applications in VANETs are governed by the duration of the
connected periods and how frequently the path between vehicles becomes
unavailable. Specifically, it can be utilized to provide information exchange
resilience by estimating an upper boundary to the amount of information that can
be exchanged between any given pair of vehicles.

In addition, the re-healing time measure is a critical metric for implementing
carry-and-forward protocols for VANETs. In these protocols, vehicles buffer the
broadcast message for some period before broadcast it to other vehicles. An
indicative  carry-and-forward protocol that has been widely used in the
literature is the VADD. Thus, re-healing time can be used to indicate the size of
message buffer and how long a vehicle should buffer the broadcast message before
it rebroadcasts it to another vehicle. Also, this metric is useful for
determining how frequently a vehicle should periodically send out the beacon
messages so that the relay vehicles can be discovered without flooding the
network. 
